Can Less be More? When Increasing-to-Balancing Label Noise Rates Considered Beneficial

In this paper, we answer the question of when inserting label noise (less informative labels) can instead return us more accurate and fair models. We are primarily inspired by three observations: 1) In contrast to reducing label noise rates, increasing the noise rates is easy to implement; 2) Increasing a certain class of instances' label noise to balance the noise rates (increasing-to-balancing) results in an easier learning problem; 3) Increasing-to-balancing improves fairness guarantees against label bias. In this paper, we first quantify the trade-offs introduced by increasing a certain group of instances' label noise rate w.r.t. the loss of label informativeness and the lowered learning difficulties. We analytically demonstrate when such an increase is beneficial, in terms of either improved generalization power or the fairness guarantees. Then we present a method to insert label noise properly for the task of learning with noisy labels, either without or with a fairness constraint. The primary technical challenge we face is due to the fact that we would not know which data instances are suffering from higher noise, and we would not have the ground truth labels to verify any possible hypothesis. We propose a detection method that informs us which group of labels might suffer from higher noise without using ground truth labels. We formally establish the effectiveness of the proposed solution and demonstrate it with extensive experiments.

==> can less be more-cr/Section/additional-experiment-result.tex <==
\section{Additional Experiment Details and Results}
We provide more details on the experimental setup as well as further results.

\subsection{Datasets}\label{app::sec::datasets}
We evaluate our methods on five datasets:
\begin{itemize}
    \item Adult, the UCI Adult Income dataset~\cite{Asuncion2007UCIML}. The task is to predict whether an individual's income exceeds 50K. The dataset consists of 48,842 examples and 28 features. We select female and male as two protected groups in constrained learning. We resample the dataset to ensure that both the classes and groups are balanced.
    \item Compas, the COMPAS recidivism dataset for crime statistics with 7,168 instances and 10 features~\cite{angwin2016machinebias}. We select race as the protected attribute in constrained learning.
    \item Fairface, the face attribute dataset containing 108,501 images with balanced race and gender groups~\cite{karkkainenfairface}. We use a pre-trained vision transformer (ViT/B-32) model~\cite{dosovitskiy2021an} to extract image representations, and project them into 50-dimensional feature vectors. For both unconstrained and constrained learning, we take gender attribute as labels for binary classification. For constrained learning, we categorize race into White and Non-White groups.
    \item MNIST~\cite{LeCun1998GradientbasedLA}, consisting of 50,000 training images and 10,000 test images in 10 classes. We train a MLP model from scratch on the MNIST dataset.
    \item CIFAR-10~\cite{Krizhevsky2009LearningML}, consisting of 50,000 training images and 10,000 test images in 10 classes. We evaluate unconstrained multi-class classification on CIFAR-10 dataset. Similar to Fairface, we use a pre-trained vision transformer to extract 512-dimensional feature vectors.
\end{itemize}

For Adult, Compas, and German datasets, we perform random train/test splits in a ratio of 80 to 20. For Fairface, MNIST, and CIFAR-10, we follow their original splits.

\subsection{Computing infrastructure}
For all the experiments, we use a GPU cluster with 4 2080 Ti GPUs for training and evaluation.

\subsection{Noise transition matrix for CIFAR-10}
We adopt the following procedure to generate the noise transition matrix: 
\begin{enumerate}
    \item Manually set the diagonal elements at least $0.4$. We ensure that the difference between the maximal elements and $0.4$ is equal to the noise gap.
    \item Permute the diagonal elements to increase the randomness.
    \item Fill out the non-diagonal elements randomly and ensure the sum of each column is 1
\end{enumerate}

We show one sample noise transition matrix generated by our procedure with noise gap $0.2$ as follows:
\[
\begin{bmatrix}
\mathbf{0.4} & 0.087 & 0.013 & 0.032 & 0.032 & 0.068 & 0.050 & 0.178 & 0.001 & 0.118 \\
0.043 & \mathbf{0.4} & 0.002 & 0.016 & 0.049 & 0.113 & 0.060 & 0.024 & 0.224 & 0.017 \\
0.181 & 0.111 & \mathbf{0.4} & 0.147 & 0.033 & 0.005 & 0.026 & 0.040 & 0.110 & 0.076 \\
0.051 & 0.001 & 0.060 & \mathbf{0.6} & 0.032 & 0.047 & 0.149 & 0.145 & 0.022 & 0.059 \\
0.001 & 0.167 & 0.119 & 0.032 & \mathbf{0.6} & 0.092 & 0.051 & 0.018 & 0.037 & 0.129 \\
0.097 & 0.007 & 0.001 & 0.059 & 0.016 & \mathbf{0.4} & 0.019 & 0.014 & 0.084 & 0.001 \\ 
0.018 & 0.023 & 0.277 & 0.041 & 0.034 & 0.014 & \mathbf{0.4} & 0.028 & 0.041 & 0.062 \\
0.149 & 0.096 & 0.081 & 0.019 & 0.041 & 0.015 & 0.143 & \mathbf{0.4} & 0.061 & 0.110 \\
0.031 & 0.066 & 0.022 & 0.007 & 0.133 & 0.080 & 0.049 & 0.113 & \mathbf{0.4} & 0.025 \\
0.029 & 0.040 & 0.023 & 0.043 & 0.027 & 0.162 & 0.048 & 0.036 & 0.018 & \mathbf{0.4}
\end{bmatrix}
\]
\subsection{Additional results}\label{app::sec::additional-results}

\begin{table}[htb]
\centering
\caption{\textbf{Binary classification accuracy of compared methods on 3 datasets across different levels of noise rates.} Mis. SL: surrogate loss~\cite{natarajan2013learning} with misspecified parameters. Est. SL: surrogate loss~\cite{natarajan2013learning} with estimated parameters. CE: vanilla cross entropy. Peer: peer loss function~\cite{liu2019peer}. 
All methods are trained with one-layer perceptron with the same hyper-parameters. For each noise setting, we average across 5 runs and report the mean and standard deviation. We find that the increasing-to-balancing can boost the vanilla cross entropy on all the noise settings.}
\label{app::table:UCI_results}
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c}
    \toprule
         & & & \multicolumn{4}{c}{\textsc{Baselines}~~(\textsc{Less Noise})} & \multicolumn{2}{c}{\ouralg ~~(\textsc{More Noise})}\\
        \cmidrule(lr){4-7}\cmidrule(lr){8-9}
         Dataset & $e_-$ & $e_+$ & \textsf{Mis. SL} & \textsf{Est. SL}  & \textsf{CE} & \textsf{Peer} & \textsf{CE} & \textsf{Peer} \\
    \midrule
        Adult & 0.0 & 0.1 & $72.79\pm0.34$ & $72.64\pm0.38$ & $72.63\pm0.29$ & $72.77\pm0.32$ & $73.62\pm0.37$ & $73.86\pm0.41$ \\
        $n = 48,842$ & 0.0 & 0.2 & $72.27\pm0.39$ & $72.13\pm0.37$ & $71.26\pm0.38$ & $71.95\pm0.34$ & $72.73\pm0.71$ & $73.52\pm0.58$ \\
        $d = 28$ & 0.0 & 0.3 & $67.93\pm0.52$ & $71.58\pm0.28$ & $66.86\pm0.47$ & $71.33\pm0.30$ & $73.30\pm0.27$ & $73.74\pm0.15$ \\
        & 0.0 & 0.4 & $55.54\pm0.28$ & $70.29\pm0.28$ & $63.97\pm1.07$ & $69.38\pm0.41$ & $73.06\pm0.50$ & $73.53\pm0.51$ \\
         & 0.1 & 0.2 & $73.02\pm0.50$ & $72.68\pm0.16$ & $72.31\pm0.25$ & $72.88\pm0.14$ & $71.92\pm1.98$ & $73.81\pm0.40$ \\
        & 0.1 & 0.3 & $72.44\pm0.47$ & $72.15\pm0.23$ & $69.06\pm2.01$ & $72.26\pm0.43$ & $69.53\pm4.90$ & $73.34\pm1.27$ \\
        & 0.1 & 0.4 & $54.87\pm0.85$ & $71.48\pm0.50$ & $63.60\pm1.04$ & $71.44\pm0.72$ & $72.43\pm1.90$ & $73.56\pm0.89$ \\
        & 0.2 & 0.3 & $72.81\pm0.51$ & $72.43\pm0.14$ & $71.44\pm0.93$ & $72.78\pm0.28$ & $71.55\pm2.04$ & $73.75\pm0.26$ \\
        & 0.2 & 0.4 & $72.06\pm0.19$ & $71.97\pm0.41$ & $63.49\pm1.58$ & $71.97\pm0.37$ & $65.99\pm7.99$ & $71.43\pm2.26$ \\
    \midrule
        Compas & 0.0 & 0.1 & $66.36\pm1.05$ & $66.04\pm1.14$ & $66.16\pm1.13$ & $68.06\pm0.70$ & $67.14\pm0.92$ & $68.22\pm0.68$ \\
        $n = 7,168$ & 0.0 & 0.2 & $66.84\pm0.69$ & $66.06\pm0.81$ & $65.38\pm1.40$ & $68.03\pm0.77$ & $66.51\pm1.90$ & $68.40\pm0.78$ \\
        $d = 10$ & 0.0 & 0.3 & $58.06\pm0.32$ & $62.69\pm1.20$ & $53.04\pm3.69$ & $66.41\pm1.19$ & $59.02\pm7.78$ & $65.93\pm0.56$ \\
        & 0.0 & 0.4 & $51.16\pm0.30$ & $62.41\pm0.71$ & $54.03\pm4.95$ & $65.01\pm0.65$ & $54.26\pm2.50$ & $65.85\pm1.17$ \\
        & 0.1 & 0.2 & $66.41\pm0.43$ & $65.69\pm0.57$ & $65.91\pm0.97$ & $67.49\pm0.40$ & $66.54\pm0.21$ & $67.80\pm0.44$ \\
        & 0.1 & 0.3 & $65.91\pm0.42$ & $65.22\pm0.63$ & $61.24\pm0.70$ & $67.36\pm0.79$ & $65.76\pm2.09$ & $68.05\pm0.56$ \\
        & 0.1 & 0.4 & $51.60\pm0.12$ & $63.34\pm1.12$ & $57.65\pm3.90$ & $66.47\pm1.34$ & $55.83\pm6.43$ & $67.04\pm0.75$ \\
        & 0.2 & 0.3 & $65.06\pm0.72$ & $65.86\pm1.69$ & $65.06\pm1.48$ & $68.02\pm0.94$ & $66.46\pm1.27$ & $68.04\pm1.11$ \\
        & 0.2 & 0.4 & $64.82\pm0.52$ & $65.47\pm0.46$ & $59.68\pm2.49$ & $67.37\pm0.54$ & $63.85\pm3.31$ & $68.39\pm0.56$ \\
    \midrule
        Fairface & 0.0 & 0.1 & $87.64\pm0.03$ & $87.75\pm0.03$ & $87.41\pm0.11$ & $87.58\pm0.15$ & $88.23\pm0.07$ & $88.49\pm0.12$ \\
        $n = 108,501$ & 0.0 & 0.2 & $85.22\pm0.06$ & $85.83\pm0.08$ & $85.08\pm0.16$ & $85.18\pm0.16$ & $88.55\pm0.03$ & $88.67\pm0.03$ \\
        $d = 50$ & 0.0 & 0.3 & $81.51\pm0.09$ & $83.36\pm0.04$ & $79.62\pm0.12$ & $81.37\pm0.35$ & $87.44\pm0.15$ & $88.25\pm0.06$ \\
        & 0.1 & 0.2 & $87.67\pm0.07$ & $87.56\pm0.04$ & $87.21\pm0.08$ & $87.28\pm0.05$ & $88.45\pm0.06$ & $88.65\pm0.07$ \\
        & 0.1 & 0.3 & $72.03\pm0.13$ & $85.68\pm0.07$ & $83.20\pm0.12$ & $84.58\pm0.09$ & $87.81\pm0.14$ & $88.50\pm0.12$ \\
        & 0.1 & 0.4 & $59.30\pm0.11$ & $83.10\pm0.08$ & $74.56\pm0.53$ & $80.51\pm0.30$ & $80.83\pm2.24$ & $87.10\pm0.39$ \\
        & 0.2 & 0.3 & $74.18\pm0.20$ & $87.34\pm0.14$ & $86.47\pm0.09$ & $87.00\pm0.11$ & $88.46\pm0.08$ & $88.58\pm0.10$ \\
        & 0.2 & 0.4 & $58.30\pm0.23$ & $85.48\pm0.09$ & $78.33\pm0.63$ & $84.05\pm0.13$ & $81.90\pm0.58$ & $87.69\pm0.15$ \\
    \bottomrule
\end{tabular}}
\end{table}

\begin{table}[!tb]
\caption{\textbf{Accuracy of compared methods across different levels of noise gap for multi-class classification.} Mis. SL: surrogate loss~\cite{natarajan2013learning} with misspecified parameters. Est. SL: surrogate loss~\cite{natarajan2013learning} with estimated parameters. CE: vanilla cross entropy. Peer: peer loss function~\cite{liu2019peer}. When noise gap is less than 0.2, cross entropy with increasing-to-balancing reaches a higher accuracy than cross entropy at a lower noise. When noise gap is 0.3, balancing cannot compensate for the loss of increasing noise.}
\label{app::table::results}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c c c c}
    \toprule
        & & \multicolumn{4}{c}{\textsc{Baselines}~~(\textsc{Less Noise})} & \multicolumn{2}{c}{\ouralg ~~(\textsc{More Noise})}\\
        \cmidrule(lr){3-6}\cmidrule(lr){7-8}
        Dataset & noise gap & \textsf{Mis. SL} & \textsf{Est. SL}  & \textsf{CE} & \textsf{Peer} & \textsf{CE} & \textsf{Peer} \\
    \midrule
        \cell{c}{MNIST} & \cell{c}{0.1 \\ 0.2 \\ 0.3} & \cell{c}{$89.59\pm0.01$ \\  $88.10\pm0.10$ \\ $84.97\pm0.11$} & \cell{c}{$89.69\pm0.07$ \\ $88.61\pm0.16$ \\ $86.88\pm0.17$} & \cell{c}{$86.66\pm0.54$ \\  $84.53\pm1.60$ \\ $85.24\pm1.05$} & \cell{c}{ $88.12\pm0.01$ \\ $87.21\pm0.53$ \\ $86.35\pm0.33$} & \cell{c}{ $86.81\pm0.62$ \\  $85.97\pm0.69$ \\  $81.89\pm1.54$} & \cell{c}{$89.19\pm0.05$ \\ $89.12\pm0.24$ \\  $88.75\pm0.19$} \\
    \midrule
          \cell{c}{CIFAR-10} & \sccell{c}{0.1 \\ 0.2 \\ 0.3} & \cell{c}{$70.90\pm2.66$ \\ $80.51 \pm 4.51$ \\ $81.30 \pm 2.31$} & \cell{c}{$85.76\pm1.44 $\\$86.34 \pm 2.30 $\\$90.61\pm0.52$} & \cell{c}{$88.03\pm1.07$ \\ $88.43\pm1.29$ \\ $89.78 \pm 1.16$} & \cell{c}{$89.66\pm1.18$ \\ $89.36 \pm 0.56$ \\ $90.24 \pm 1.05$} & \cell{c}{$88.69\pm0.82$ \\ $89.01 \pm 1.27$ \\ $87.98\pm1.29$} & \cell{c}{$89.90\pm0.52$ \\ $90.08 \pm 1.26$ \\ $89.92 \pm 0.92$} \\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[tb]
    \newcommand{\metric}[0]{\textit{accuracy} \\ \textit{fairness}}
    \centering
    \caption{\textbf{Constrained learning results with group-dependent label noise.} LR: na\"ive logistic regression without noise correction. GPR: group-weighted peer loss~\cite{wang2021fair}. Peer: peer loss~\cite{liu2019peer}.}
    \label{app::table::fairness_results}
    \begin{tabular}{l c c c c c c c}
    \toprule
         & & & & \multicolumn{2}{c}{\textsc{Less Noise}} & \multicolumn{2}{c}{\textsc{More Noise}}\\
        \cmidrule(lr){5-6}\cmidrule(lr){7-8}
         Dataset & $e_a$ & $e_b$ & Metrics & \textsf{LR} & \textsf{GPL} & \textsf{LR} & \textsf{Peer} \\
    \midrule
        \cell{c}{Adult} & \cell{c}{0.1 \\ \\ 0.2 \\ \\ 0.2 \\ \\ 0.3 \\} & \cell{c}{0.3\\ \\ 0.3 \\ \\ 0.4 \\ \\ 0.4\\} & \cell{c}{\metric \\ \metric \\ \metric \\ \metric\\} & \cell{c}{72.57 \\ 2.37 \\ 72.4 \\ 6.67 \\ 72.73 \\ 6.48 \\ 73.15 \\ 5.29 \\} & \cell{c}{71.92 \\ 3.39 \\ 72.92 \\ 3.36 \\ 71.2 \\ 2.95 \\ 73.74 \\ 4.11\\ } & \cell{c}{71.07 \\ 1.83 \\ 73.07 \\ 4.21 \\ 71.88 \\ 3.16 \\ 71.36 \\ 5.49 \\} & \cell{c}{73.21 \\ 1.95 \\ 71.8 \\ 0.93 \\ 73.02 \\ 1.67 \\ 72.74 \\ 1.88} \\
    \midrule
        \cell{c}{Compas} & \cell{c}{0.1 \\ \\ 0.2 \\ \\ 0.2 \\ \\ 0.3 \\} & \cell{c}{0.3\\ \\ 0.3 \\ \\ 0.4 \\ \\ 0.4\\} & \cell{c}{\metric \\ \metric \\ \metric \\ \metric} & \cell{c}{63.88 \\ 7.17 \\ 63.73 \\ 10.52 \\ 62.60 \\ 2.87 \\ 61.93 \\ 17.97 \\} & \cell{c}{ 63.73 \\ 6.58 \\ 63.28 \\ 4.47 \\ 66.03 \\ 7.55 \\ 62.08 \\ 3.06 \\} & \cell{c}{ 64.56 \\ 7.35 \\ 64.26 \\ 7.10 \\ 66.22 \\ 6.07 \\ 61.63 \\ 7.70 \\} & \cell{c}{64.33 \\ 1.89 \\ 67.8\\ 2.76 \\ 64.15 \\ 3.63 \\ 62.68 \\ 3.74 \\} \\
    \midrule
        \cell{c}{Fairface} & \cell{c}{0.2 \\ \\ 0.1 \\ \\ 0.0\\ \\ 0.0 \\ \\ 0.2 \\} & \cell{c}{0.4 \\ \\ 0.3 \\ \\ 0.2 \\ \\ 0.1 \\ \\ 0.3 \\} & \cell{c}{\metric \\ \metric \\ \metric \\ \metric \\ \metric } & \cell{c}{86.97 \\ 5.87 \\ 88.23 \\ 5.53 \\ 88.61 \\ 4.05 \\ 89.08 \\ 3.99 \\ 88.63 \\ 3.50} & \cell{c}{87.47 \\ 4.70 \\ 88.23\\ 4.93 \\ 88.53 \\ 3.75 \\ 88.84 \\ 3.92 \\ 88.78 \\ 3.14} & \cell{c}{88.19 \\ 1.38 \\ 88.58 \\ 2.11 \\ 88.90 \\ 2.64 \\ 89.00 \\ 2.97 \\ 88.80 \\ 2.19} & \cell{c}{87.93 \\ 0.25 \\ 88.60 \\ 2.17 \\ 88.85 \\ 2.20 \\ 89.05 \\ 2.91 \\ 88.83 \\ 1.33 \\} \\
    \bottomrule
    \end{tabular}
\end{table}

==> can less be more-cr/Section/experiment.tex <==
In order to verify the power of our increasing-to-balancing method, we conduct extensive experiments on both unconstrained learning and constrained learning settings. The datasets include: the UCI Adult Income dataset~\cite{Asuncion2007UCIML}, the Compas recidivism dataset~\cite{angwin2016machinebias}, Fairface~\cite{karkkainenfairface} face attribute dataset, and CIFAR 10~\cite{Krizhevsky2009LearningML} dataset. We defer more dataset details to Appendix \ref{app::sec::datasets}.

\begin{table}[!tb]
\definecolor{best}{HTML}{BAFFCD}
\definecolor{issue}{HTML}{FFC8BA}
\definecolor{better}{HTML}{BBDDFF}
\newcommand{\good}[1]{\cellcolor{best}#1} 
\newcommand{\bad}[1]{\cellcolor{issue}#1} 
\newcommand{\better}[1]{\cellcolor{better}#1} 
\centering
\caption{\textbf{Binary classification accuracy of compared methods on 3 datasets across different levels of noise rates.} Mis. SL: surrogate loss~\cite{natarajan2013learning} with misspecified parameters. Est. SL: surrogate loss~\cite{natarajan2013learning} with estimated parameters. CE: vanilla cross entropy. Peer: peer loss function~\cite{liu2019peer}. 
All methods are trained with one-layer perceptron with the same hyper-parameters. For each noise setting, we average across 5 runs and report the mean and standard deviation. We find that the increasing-to-balancing can boost the vanilla cross entropy on all the noise settings. We highlight any boost of increasing-to-balancing for vanilla CE in green, and the best accuracy in blue.}
\label{table:UCI_results}
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c}
    \toprule
         & & & \multicolumn{4}{c}{\textsc{Baselines}~~(\textsc{Less Noise})} & \multicolumn{2}{c}{\ouralg ~~(\textsc{More Noise})}\\
        \cmidrule(lr){4-7}\cmidrule(lr){8-9}
         Dataset & $e_-$ & $e_+$ & \textsf{Mis. SL} & \textsf{Est. SL}  & \textsf{CE} & \textsf{Peer} & \textsf{CE} & \textsf{Peer} \\
    \midrule
        Adult & 0.0 & 0.1 & $72.79\pm0.34$ & $72.64\pm0.38$ & $72.63\pm0.29$ & $72.77\pm0.32$ & \good{$73.62\pm0.37$} & \better{$73.86\pm0.41$} \\
        $n = 48,842$ & 0.0 & 0.2 & $72.27\pm0.39$ & $72.13\pm0.37$ & $71.26\pm0.38$ & $71.95\pm0.34$ & \good{$72.73\pm0.71$} & \better{$73.52\pm0.58$} \\
        $d = 28$ & 0.1 & 0.2 & $73.02\pm0.50$ & $72.68\pm0.16$ & $72.31\pm0.25$ & $72.88\pm0.14$ & $71.92\pm1.98$ & \better{$73.81\pm0.40$} \\
        & 0.1 & 0.3 & $72.44\pm0.47$ & $72.15\pm0.23$ & $69.06\pm2.01$ & $72.26\pm0.43$ & \good{$69.53\pm4.90$} & \better{$73.34\pm1.27$} \\
        & 0.2 & 0.3 & $72.81\pm0.51$ & $72.43\pm0.14$ & $71.44\pm0.93$ & $72.78\pm0.28$ & \good{$71.55\pm2.04$} & \better{$73.75\pm0.26$} \\
        & 0.2 & 0.4 & \better{$72.06\pm0.19$} & $71.97\pm0.41$ & $63.49\pm1.58$ & $71.97\pm0.37$ & \good{$65.99\pm7.99$} & $71.43\pm2.26$ \\
        & 0.3 & 0.4 & $52.65\pm0.53$ & $72.67\pm0.26$ & $71.55\pm0.88$ & $73.49\pm0.18$ & \good{$72.54\pm1.84$} & \better{$74.27\pm0.20$} \\
    \midrule
        Compas & 0.0 & 0.1 & $66.36\pm1.05$ & $66.04\pm1.14$ & $66.16\pm1.13$ & $68.06\pm0.70$ & \good{$67.14\pm0.92$} & \better{$68.22\pm0.68$} \\
        $n = 7,168$ & 0.0 & 0.2 & $66.84\pm0.69$ & $66.06\pm0.81$ & $65.38\pm1.40$ & $68.03\pm0.77$ & \good{$66.51\pm1.90$} & \better{$68.40\pm0.78$} \\
        $d = 10$ & 0.1 & 0.2 & $66.41\pm0.43$ & $65.69\pm0.57$ & $65.91\pm0.97$ & $67.49\pm0.40$ & \good{$66.54\pm0.21$} & \better{$67.80\pm0.44$} \\
        & 0.1 & 0.3 & $65.91\pm0.42$ & $65.22\pm0.63$ & $61.24\pm0.70$ & $67.36\pm0.79$ & \good{$65.76\pm2.09$} & \better{$68.05\pm0.56$} \\
        & 0.2 & 0.3 & $65.06\pm0.72$ & $65.86\pm1.69$ & $65.06\pm1.48$ & $68.02\pm0.94$ & \good{$66.46\pm1.27$} & \better{$68.04\pm1.11$} \\
        & 0.2 & 0.4 & $64.82\pm0.52$ & $65.47\pm0.46$ & $59.68\pm2.49$ & $67.37\pm0.54$ & \good{$63.85\pm3.31$} & \better{$68.39\pm0.56$} \\
    \midrule
        Fairface & 0.0 & 0.1 & $87.64\pm0.03$ & $87.75\pm0.03$ & $87.41\pm0.11$ & $87.58\pm0.15$ & \good{$88.23\pm0.07$} & \better{$88.49\pm0.12$} \\
        $n = 108,501$ & 0.0 & 0.2 & $85.22\pm0.06$ & $85.83\pm0.08$ & $85.08\pm0.16$ & $85.18\pm0.16$ & \good{$88.55\pm0.03$} & \better{$88.67\pm0.03$} \\
        $d=50$ & 0.1 & 0.2 & $87.67\pm0.07$ & $87.56\pm0.04$ & $87.21\pm0.08$ & $87.28\pm0.05$ & \good{$88.45\pm0.06$} & \better{$88.65\pm0.07$} \\
        & 0.1 & 0.3 & $72.03\pm0.13$ & $85.68\pm0.07$ & $83.20\pm0.12$ & $84.58\pm0.09$ & \good{$87.81\pm0.14$} & \better{$88.50\pm0.12$} \\
        & 0.2 & 0.3 & $74.18\pm0.20$ & $87.34\pm0.14$ & $86.47\pm0.09$ & $87.00\pm0.11$ & \good{$88.46\pm0.08$} & \better{$88.58\pm0.10$} \\
        & 0.2 & 0.4 & $58.30\pm0.23$ & $85.48\pm0.09$ & $78.33\pm0.63$ & $84.05\pm0.13$ & \good{$81.90\pm0.58$} & \better{$87.69\pm0.15$} \\
    \bottomrule
\end{tabular}}
\vspace{-0.1in}
\end{table}
\subsection{Unconstrained learning}
\textbf{Setup.} For the unconstrained learning, we implement a one-layer perceptron for binary classification on Adult, Compas, and Fairface datasets. We flip the true labels on training set according to a set of asymmetric noise rates, train the models on the corrupted labels, and evaluate the accuracy on test set with clean labels. The baseline methods we compare include: surrogate loss~\cite{natarajan2013learning} with mis-specified noise rates (\textbf{Mis. SL}) and estimated noise rates (\textbf{Est. SL}) respectively, vanilla cross entropy (\textbf{CE}), and peer loss functions~\cite{liu2019peer} (\textbf{Peer}). For Mis. SL, we randomly generate the noise parameters but ensure that the trace is equal to that of the true noise transition matrix. For Est. SL, we estimate the noise rates by adopting the confident learning procedure~\cite{northcutt2021confident}. We note that the training of peer loss functions does not require the knowledge of noise rates, and follow their instructions to tune the hyper-parameters through cross-validation. For the same corrupted training labels, we deploy our increasing-to-balancing procedure, and evaluate the performance of cross entropy and peer loss functions again. We set the threshold $\gamma$ used in Algorithm \ref{alg:noise++} as $0.1\%$ on Adult and Fairface datasets, and loose it to $1\%$ on Compas due to its much smaller data size. We repeat all the methods 5 runs with different random seeds and report the mean and standard deviation.

\textbf{Results.} We show the experimental results in Table \ref{table:UCI_results}. We observe that our increasing-to-balancing method significantly improves the accuracy of the vanilla cross entropy on the majority of noise settings. It is notable that the cross entropy with increasing-to-balancing has a comparable performance with Est. SL, when the noise is relatively small. When the noise rates are large (e.g. 0.2 and 0.4), we observe a significant degradation for cross entropy, but increasing-to-balancing still boosts the accuracy. Moreover, we find that peer loss after increasing-to-balancing is more robust to noise, and dominantly achieve the highest accuracy.

\vspace{0.05in}
\begin{minipage}[!tb]{\textwidth}
\begin{minipage}[b]{0.65\linewidth}
\definecolor{best}{HTML}{BAFFCD}
\definecolor{issue}{HTML}{FFC8BA}
\definecolor{bad}{HTML}{FFA500}
\newcommand{\good}[1]{\cellcolor{best}#1} 
\newcommand{\bad}[1]{\cellcolor{issue}#1} 
\newcommand{\better}[1]{\cellcolor{bad}#1} 
\captionsetup{type=table}
\caption{\textbf{Accuracy of compared methods across different levels of noise gap for multi-class classification.}}
\label{table:multi-class}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l c c c c c c c}
    \toprule
        & & \multicolumn{4}{c}{\textsc{Less Noise}} & \multicolumn{2}{c}{\textsc{More Noise}}\\
        \cmidrule(lr){3-6}\cmidrule(lr){7-8}
        Dataset & noise gap & \textsf{Mis. SL} & \textsf{Est. SL}  & \textsf{CE} & \textsf{Peer} & \textsf{CE} & \textsf{Peer} \\
    \midrule
        \cell{c}{MNIST} & \cell{c}{0.1 \\ 0.2 \\ 0.3} & \cell{c}{89.59 \\ 88.10 \\ 84.97} & \cell{c}{89.69 \\ 88.61 \\ 86.88} & \cell{c}{86.66 \\ 84.53 \\ 85.24} & \cell{c}{88.12 \\ 87.21 \\ 86.35} & \cell{c}{\good{86.81} \\ \good{85.97} \\ \bad{81.89}} & \cell{c}{89.19 \\ 89.12 \\ 88.75} \\
    \midrule
        \cell{c}{CIFAR-10} & \cell{c}{0.1 \\ 0.2 \\ 0.3} & \cell{c}{$70.90$ \\ $80.51$ \\ $81.30$} & \cell{c}{$85.76 $\\$86.34$\\$90.61$} & \cell{c}{$88.03$ \\ $88.43$ \\ $89.78$} & \cell{c}{$89.66$ \\ $89.36$ \\ $90.24$} & \cell{c}{\good{$88.69$} \\ \good{$89.01$} \\ \bad{$87.98$}} & \cell{c}{$89.90$ \\ $90.08$ \\ $89.92$} \\
    \bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}[b]{0.3\linewidth}
\captionsetup{type=table}
\caption{\textbf{Accuracy of compared methods on Clothing1M dataset.}}
\label{table:clothing1m}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l c}
    \toprule
        Method & Test Accuracy  \\
    \midrule
        CE & $68.94\%$ \\
        Loss Correction~\cite{patrini2017making} & $69.84\%$ \\
        Co-Teaching~\cite{han2018co} & $70.15\%$ \\
        CE + \ouralg &  $\mathbf{70.37\%}$ \\
    \bottomrule
\end{tabular}}
\end{minipage}
\end{minipage}
\vspace{0.05in}

\textbf{Multi-class extension.} We test \ouralg{} in the multi-class setting by balancing the noise rates class by class. We evaluate the compared methods on MNIST~\cite{LeCun1998GradientbasedLA} and CIFAR-10~\cite{Krizhevsky2009LearningML} with more sophisticated noise transition matrices. Considering that both datasets have 10 classes, we adopt the following procedure to generate the $10\times10$ noise transition matrix: (1) manually set the diagonal elements at least $0.4$; (2) permute the diagonal elements to increase the randomness; (3) fill out the non-diagonal elements randomly and ensure the sum of each column is 1. An MLP model is trained from scratch on MNIST dataset, while a pre-trained vision transformer~\cite{dosovitskiy2021an} is used to extract visual features on CIFAR-10 dataset. As shown in Table \ref{table:multi-class}, we observe that when the noise gap is $0.1$ and $0.2$, CE and Peer with \ouralg{} outperforms the pure CE and Peer, respectively. When the noise gap is $0.3$, balancing cannot compensate for the performance drop due to increased noise.

\textbf{Experiments on Clothing1M.} Clothing1M is a large-scale dataset collected from online shopping websites, comprising of 1 million training images of clothes with realistic noisy and 10,000 test data with clean labels. For a fair comparison, we adopted the same setting as described in \cite{patrini2017making} and trained a ResNet-50~\cite{he2016deep} classifier. Table \ref{table:clothing1m} compares our methods with some other baselines, including loss correction~\cite{patrini2017making} and Co-Teaching~\cite{han2018co}. Without a careful tuning of training parameters, vanilla CE with \ouralg reached $70.37\%$ test accuracy. In comparison, standard CE achieves $68.94\%$, loss correction achieves $69.84\%$, and Co-Teaching is $70.15\%$.

\subsection{Constrained learning}
\begin{table}[!t]
    \definecolor{good}{HTML}{BAFFCD}
    \newcommand{\good}[1]{\cellcolor{good}#1} 
    \newcommand{\metric}[0]{\textit{accuracy} \\ \textit{fairness}}
    \centering
    \caption{\textbf{Constrained learning results with group-dependent label noise.} We only report the results for $e_a = 0.2$ and $e_b = 0.4$. LR: na\"ive logistic regression without noise correction. GPR: group-weighted peer loss~\cite{wang2021fair}. Peer: peer loss~\cite{liu2019peer}. We highlight numbers of low fairness violation.}
    \label{tab:fairness_results}
    \resizebox{!}{!}{
    \begin{tabular}{l c c c c c}
    \toprule
         & & \multicolumn{2}{c}{\textsc{Less Noise}} & \multicolumn{2}{c}{\textsc{More Noise}}\\
        \cmidrule(lr){3-4}\cmidrule(lr){5-6}
         Dataset & Metrics & \textsf{LR} & \textsf{GPL} & \textsf{LR} & \textsf{Peer} \\
    \midrule
        \cell{c}{Adult} & \cell{c}{\metric} & \cell{c}{72.73 \\ 6.48 \\} & \cell{c}{71.2 \\ \good{2.95} \\ } & \cell{c}{ 71.88 \\ \good{3.16} \\ } & \cell{c}{ 73.02 \\ \good{1.67} \\} \\
        \cell{c}{Compas} & \cell{c}{\metric} & \cell{c}{62.60 \\ \good{2.87} \\} & \cell{c}{66.03 \\ 7.55} & \cell{c}{66.22 \\ 6.07 \\} & \cell{c}{64.15 \\ \good{3.63} \\} \\        
        \cell{c}{Fairface} & \cell{c}{\metric} & \cell{c}{86.97 \\ 5.87 \\} & \cell{c}{87.47 \\ 4.70 \\} & \cell{c}{88.19 \\ \good{1.38}} & \cell{c}{87.93 \\ \good{0.25} \\} \\
    \bottomrule
    \end{tabular}}
    \vspace{-0.1in}
\end{table}
\textbf{Setup.} We conduct experiments with equal odds constraints~\cite{hardt2016equalodds} on Adult, Compas, and Fairface datasets. We add heterogeneous noise, i.e., uneven noise rates for different group memberships but symmetric for different classes, into training labels but keep test labels clean. We stress-test the performance of the na\"ive logistic regression (LR) and group-weighted peer loss (GPL)~\cite{wang2021fair} with and without our increasing-to-balancing program.\footnote{We did not repeat testing surrogate loss as it is reported in \cite{wang2021fair} that GPL appears to be a better and more robust solution. Also we focus on correcting fairness constraints in this section, both SL and GPL would use the same constraint corrections.} We note that GPL degrades to peer loss when noise rates are homogeneous across protected groups~\cite{wang2021fair}, and directly apply peer loss after balancing. For a fair comparison, we use logistic regression as the base classifier for all the methods. We use the reductions approach~\cite{pmlr-v80-agarwal18a} to solve the constrained optimization.

\textbf{Results.} We report the accuracy and fairness violation for $e_a = 0.2$ and $e_b = 0.4$ in Table~\ref{tab:fairness_results} and defer more noise settings to Appendix~\ref{app::sec::additional-results}. We make the following observations: (1) All the methods retain a comparable accuracy. We conjecture that this benefits from the symmetric noise rates between positive and negative classes. (2) After balancing, both na\"ive LR and Peer significantly mitigate the fairness violations on Adult and Fairface datasets as a result of equalized noise rates across groups. (3) Peer loss generally has a lower fairness violation than na\"ive LR. This implies its capability of recovering unbiased classifiers. (4) We find out that the performance of LR with increasing-to-balancing is less profitable on Compas dataset because of uninformative features (only 10-dimensional features), and more robust on Fairface dataset with rich image information.


==> can less be more-cr/Section/proofs.tex <==
\makeSupplementaryMaterialTitle

This Appendix is organized as follows:
\squishlist
\item Section A includes omitted proofs for theoretical conclusions in the main paper, as well as the extension to fairness constrained setting (\ref{app:sec::balance-for-fairness}) and multi-class classification (\ref{app::sec::estimate-multiclass}).
\item Section B presents more experimental details and results.
\squishend
\section{Omitted Proofs}
\subsection{Proof for Theorem \ref{thm:r:sl}}
\label{app:1}
\begin{proof}
Let $\lc$ denote the noise-corrected loss with respect to true noise parameters $e_+,e_-$:
\begin{align}
    \lc(h(x_n),\ny_n):= (1-e_{-sgn(\ny_n)})\cdot \ell(h(x_n),\ny_n) - e_{sgn(\ny_n)} \cdot  \ell(h(x_n),-\ny_n)
\end{align}
It was established in \cite{natarajan2013learning} the unbiasedness of $\lc$:
\begin{lemma}[Unbiasedness of $\lc$,~\cite{natarajan2013learning}]
$\frac{1}{1-e_+-e_-} \cdot \mathbb E_{\tilde{Y}|Y=y}[ \lc(h(x),\nY)] = \ell(h(x),y).$
\end{lemma}
A direct consequence of this lemma, via repeatedly applying to each $(X,Y)$, is its unbiasedness on the population level:
\[
\frac{1}{1-e_+-e_-}\cdot  \mathbb E_{\tilde{D}|D}[\hat{R}_{\lc,\tilde{D}}(h)] =  \hat{R}_{\ell,D}(h),~~~\frac{1}{1-e_+-e_-}\cdot R_{\lc,\tilde{\D}}(h) =  R_{\ell,\D}(h)
\]

The following fact holds by subtracting $\lc$ from $\lce$:
\begin{align*}
    \lce(h(x_n),\tilde{y}_n) &= \lc(h(x_n),\tilde{y}_n)
    + (e_{-\tilde{y}_n}-\tilde{e}_{-\tilde{y}_n})\cdot \ell(h(x_n),\tilde{y}_n)
    + (\tilde{e}_{-\tilde{y}_n}-e_{\tilde{y}_n})\cdot \ell(h(x_n),-\tilde{y}_n)
\end{align*}
Using the triangle inequality of $|\cdot|$ we establish that
\begin{align}
    |\lce(h(x_n),\tilde{y}_n) - \lc(h(x_n),\tilde{y}_n)| \leq \max\{|\nep - e_+|,|\nen-e_-|\} \cdot \bar{\ell}.
\end{align}
This further helps us bound the differences in the empirical risks:
\begin{align}
   |\hat{R}_{\lce,\tilde{D}}(h) - \hat{R}_{\lc,\tilde{D}}(h)| \leq  \max\{|\nep - e_+|,|\nen-e_-|\} \cdot \bar{\ell}
\end{align}
Therefore 
\begin{align}
\hat{R}_{\lc,\tilde{D}}(h^*_{\lce,\tilde{D}} ) &\leq \hat{R}_{\lce,\tilde{D}}(h^*_{\lce,\tilde{D}} ) + \max\{|\nep - e_+|,|\nen-e_-|\} \cdot \bar{\ell}\nonumber \\
&\leq \hat{R}_{\lce,\tilde{D}}(h^{*}_{\ell,\D})+ \max\{|\nep - e_+|,|\nen-e_-|\} \cdot \bar{\ell}\tag{\text{Opt. of $h^*_{\ell,\hat{D}}$}}\\
&\leq \hat{R}_{\lc,\tilde{D}}(h^{*}_{\ell,\D})+ 2\max\{|\nep - e_+|,|\nen-e_-|\} \cdot \bar{\ell}\label{eqn:thm1:bd1}
\end{align}
Calling the results in \cite{natarajan2013learning}, [Rademacher bound for max risk deviation, Proof of Lemma 2 therein], we know that for any $\delta>0$, with probability at least $1-\delta$:
\begin{align}
\sup_{h \in \H}  \frac{1}{1-e_+-e_-}\left| R_{\lc,\nD}(h) - \hat{R}_{\lc,\tilde{D}}(h)\right| \leq \frac{2L}{1-e_+-e_-}\cdot \RR(\H) + \sqrt{\frac{\log 1/\delta}{2N}}\label{bd:rad}
\end{align}
The above knowledge further helps us establish that 
\begin{align*}
    &\ \ R_{\ell,\D}(h^*_{\lce,\tilde{D}} )-  R_{\ell,\D}(h^{*}_{\ell,\D})\\
    =&\ \ \frac{1}{1-e_+-e_-} (R_{\lc,\nD}(h^*_{\lce,\tilde{D}} )-  R_{\lc,\nD}(h^{*}_{\ell,\D})) \tag{\text{Unbiasedness of $\lc$ on $\nD$}}\\
    =&\ \ \frac{1}{1-e_+-e_-}(R_{\lc,\nD}(h^*_{\lce,\tilde{D}} ) - \hat{R}_{\lc,\tilde{D}}(h^*_{\lce,\tilde{D}} )) \tag{\text{Rademacher bound }}\\
    &\ + \frac{1}{1-e_+-e_-}(\hat{R}_{\lc,\tilde{D}}(h^*_{\lce,\tilde{D}} ) -  \hat{R}_{\lc,\tilde{D}}(h^{*}_{\ell,\D}))\tag{Eqn. (\ref{eqn:thm1:bd1})}\\
    &\ +\frac{1}{1-e_+-e_-}(\hat{R}_{\lc,\tilde{D}}(h^{*}_{\ell,\D}) - R_{\lc,\nD}(h^{*}_{\ell,\D}))\tag{\text{Rademacher bound }}\\
    \leq &\ \ \frac{4L}{1-e_+-e_-}\cdot \RR(\H) + 2\sqrt{\frac{\log 1/\delta}{2N}}+ 2\frac{\max\{|\nep - e_+|,|\nen-e_-|\}}{1-e_+-e_-} \cdot \bar{\ell}\\
    \leq &\ \ \frac{4L}{1-e_+-e_-}\cdot \RR(\H) + 2\sqrt{\frac{\log 1/\delta}{2N}} + 2\frac{\errm}{1-e_+-e_-} \cdot \bar{\ell}~.
\end{align*}
We complete the proof. 
\end{proof}

\subsection{Proof for Lemma \ref{lemma:balance:e}}
\begin{proof}
Expanding $\P(h(X) \neq \hat{Y})$ using the law of total probability we have
\begin{align*}
    \P(h(X) \neq \hat{Y}) 
    =&\ \ \P(h(X) \neq \hat{Y},\hat{Y} \neq Y) + \P(h(X) \neq \hat{Y},\hat{Y} = Y)\\
    =&\ \ \P(h(X) \neq \hat{Y}\mid\hat{Y} \neq Y)\cdot \P(\hat{Y} \neq Y) +\P(h(X) \neq \hat{Y}\mid\hat{Y} = Y) \cdot \P(\hat{Y} = Y).~
\end{align*}
In binary classification, $h(X) \neq \nY, \nY \neq Y$ implies $h(X) = Y$, such that
\[
\P(h(X) \neq \nY \mid \nY \neq Y) = \P(h(X) = Y \mid \nY \neq Y).~
\]
Due to the independence of $\nY$ and $X$ given $Y$,
\[
 \P(h(X) = Y \mid \nY \neq Y) = \frac{\P(h(X) = Y, \nY \neq Y)}{\P(\nY \neq Y)} = \frac{\P(h(X) = Y)\P(\nY \neq Y)}{\P(\nY \neq Y)} = \P(h(X) = Y)
\]
Similarly, we have
\[
\P(h(X) \neq \hat{Y}\mid\hat{Y} = Y) = \P(h(X) \neq \nY).~
\]
Combining all above we finished the proof when $e<0.5$ by having:
\begin{align*}
    \P(h(X) \neq \hat{Y}) = &\ \ \P(h(X) = Y)\cdot e + \P(h(X) \neq Y) \cdot (1-e)\\
    = &\ \ (1-2e) \cdot \P(h(X) \neq Y) + e
\end{align*}
\end{proof}
\subsection{Proof for Theorem \ref{thm:r:symmetric}}

\begin{proof}
Again let $\lc$ denote the noise-corrected loss with respect to true noise parameters $e_+,e_-$:
\begin{align}
    \lc(h(x_n),\ny_n):= (1-e_{-sgn(\ny_n)})\cdot \ell(h(x_n),\ny_n) - e_{sgn(\ny_n)} \cdot  \ell(h(x_n),-\ny_n)
\end{align}
First notice the following when $\ell$ is a symmetric loss:
\begin{align}
    &\ \ R_{\ell,\D}(h^*_{\ell,\hat{D}}) \nonumber \\
    =&\ \ \frac{1}{1-2e} \cdot R_{\lc,\hat{\D}}(h^*_{\ell,\hat{D}}) \tag{\text{Unbiasedness of $\lc$ on $\hat{\D}$} using symmetric $e$}\\
    =&\ \ \frac{1-e}{1-2e}\cdot  R_{\ell,\hat{\D}}(h^*_{\ell,\hat{D}})-\frac{e}{1-2e} \cdot R_{\ell,\hat{\D}}(-h^*_{\ell,\hat{D}}) \label{eqn:unbias}
\end{align}
The last equality uses the definition of $\lc$, and is due to $\ell$ being symmetric. Then we show that
\begin{align*}
    &\ \ \frac{1}{1-2e} \cdot \left(R_{\ell,\hat{\D}}(h^*_{\ell,\hat{D}}) - R_{\ell,\hat{\D}}(h^{*}_{\ell,\D})\right)\\
    =&\ \ \frac{1}{1-2e}\left(R_{\ell,\hat{\D}}(h^*_{\ell,\hat{D}}) - \hat{R}_{\ell,\hat{D}}(h^*_{\ell,\hat{D}})\right)\tag{\text{Rademacher bound }}\\
    &\ + \frac{1}{1-2e}\left(\hat{R}_{\ell,\hat{D}}(h^*_{\ell,\hat{D}}) -  \hat{R}_{\ell,\hat{D}}(h^{*}_{\ell,\D})\right)\tag{$\leq$ 0~~\text{Optimality of $h^*_{\lce,\hat{D}} $ on $\ell,\hat{D}$}}\\
    &\ +\frac{1}{1-2e}\left(\hat{R}_{\ell,\hat{D}}(h^{*}_{\ell,\D}) - R_{\ell,\hat{\D}}(h^{*}_{\ell,\D})\right)\tag{\text{Rademacher bound }}\\
    \leq &\ \ \frac{4L}{1-2e}\RR(\H) + 2\sqrt{\frac{\log 1/\delta}{2N}}
\end{align*}
The inequality is due to the Rademacher bound we invoked as in Eqn. (\ref{bd:rad}) as well as the optimality of $h^*_{\ell,\hat{D}}$ on $\ell,\hat{D}$. That is we have proved with probability at least $1-\delta$ that
\begin{align}\label{thm3:bd1}
     \frac{1}{1-2e} \cdot R_{\ell,\hat{\D}}(h^*_{\ell,\hat{D}}) \leq \frac{1}{1-2e} \cdot R_{\ell,\hat{\D}}(h^{*}_{\ell,\D}) + \frac{4L}{1-2e}\RR(\H) + 2\sqrt{\frac{\log 1/\delta}{2N}}
\end{align}
Repeating the same analysis and using the assumed condition that $\hat{R}_{\ell,\hat{D}}(-h^*_{\ell,\hat{D}}) -  \hat{R}_{\ell,\hat{D}}(-h^{*}_{\ell,\D}) \geq 0$ we have
\begin{align}\label{thm3:bd2}
     \frac{1}{1-2e} \cdot R_{\ell,\hat{\D}}(-h^*_{\ell,\hat{D}}) \geq \frac{1}{1-2e} \cdot R_{\ell,\hat{\D}}(-h^{*}_{\ell,\D}) - \frac{4L}{1-2e}\RR(\H) - 2\sqrt{\frac{\log 1/\delta}{2N}}
\end{align}
Combining above (Eqn. (\ref{thm3:bd1}) and (\ref{thm3:bd2})), we have with probability at least $1-\delta$ (that both of the above bounds will happen simultaneously)
\begin{align*}
    R_{\ell,\D}(h^*_{\ell,\hat{D}}) = &\ \ \frac{1-e}{1-2e} \cdot R_{\ell,\hat{\D}}(h^*_{\ell,\hat{D}})-\frac{e}{1-2e} \cdot R_{\ell,\hat{\D}}(-h^*_{\ell,\hat{D}})\\
    \leq &\ \ \frac{1-e}{1-2e} \cdot R_{\ell,\hat{\D}}(h^{*}_{\ell,\D})-\frac{e}{1-2e} \cdot R_{\ell,\hat{\D}}(-h^{*}_{\ell,\D}) + \frac{4L}{1-2e}\RR(\H) + 2\sqrt{\frac{\log 1/\delta}{2N}}\\
    =&\ \ R_{\ell,\D}(h^{*}_{\ell,\D}) + \frac{4L}{1-2e}\RR(\H) + 2\sqrt{\frac{\log 1/\delta}{2N}}.
\end{align*}
The inequality uses Eqn. (\ref{thm3:bd1}) and (\ref{thm3:bd2}). Again the last equality is reusing Eqn. (\ref{eqn:unbias}).
This completes the proof. 
\end{proof}

\subsection{Proof for Lemma \ref{lemma:constraint}}

\begin{proof}
\begin{align}
    \P(h(X)=+1|\tilde{Y}=+1,Z=a) = \frac{\P(h(X)=+1,\tilde{Y}=+1|Z=a)}{\P(\tilde{Y}=+1|Z=a)}
\end{align}
Again we do the trick of sampling $\P(\tilde{Y}=+1|Z=a)$ to be 0.5, which allows us to focus on the numerator. 
\begin{align*}
    &\ \ \P(h(X)=+1,\tilde{Y}=+1|Z=a) \\
    = &\ \ \P(h(X)=+1,\tilde{Y}=+1, Y=+1|Z=a) \\
    &\ + \P(h(X)=+1,\tilde{Y}=+1, Y=-1|Z=a)\\
    =&\ \ \P(h(X)=+1,\tilde{Y}=+1|Y=+1,Z=a) \cdot \P(Y=+1|Z=a)\\
    &\ + \P(h(X)=+1,\tilde{Y}=+1|Y=-1,Z=a)\cdot \P(Y=-1|Z=a)\\
    =&\ \ \P(h(X)=+1|Y=+1,Z=a) \cdot (1-e_a) \cdot \P(Y=+1|Z=a)\\
    &\ + \P(h(X)=+1|Y=-1,Z=a)\cdot e_a \cdot \P(Y=-1|Z=a)\tag{\text{Independence of $X$ and $\tilde{Y}$ given $Y$}}
\end{align*}
That is
\begin{align}
    0.5 \cdot \nTPR_a(h) = \TPR_a(h) \cdot (1-e_a) \cdot \P(Y=+1|Z=a) + \FPR_a(h) \cdot e_a \cdot \P(Y=-1|Z=a)\label{eqn:tpr}
\end{align}
Similarly for FPR we have
\begin{align}
    \P(h(X)=+1|\tilde{Y}=-1,Z=a) = \frac{\P(h(X)=+1,\tilde{Y}=-1|Z=a)}{\P(\tilde{Y}=-1|Z=a)}
\end{align}
Following similar steps as above, the numerator further derives as
\begin{align*}
    &\ \ \P(h(X)=+1,\tilde{Y}=+1|Z=a) \\
   =&\ \ \P(h(X)=+1|Y=-1,Z=a) \cdot (1-e_a) \cdot \P(Y=+1|Z=a)\\
    &\ + \P(h(X)=+1|Y=+1,Z=a)\cdot e_a \cdot \P(Y=-1|Z=a)
\end{align*}
That is 
\begin{align}
    0.5 \cdot \nFPR_a(h) = \FPR_a(h) \cdot (1-e_a) \cdot \P(Y=+1|Z=a) + \TPR_a(h) \cdot e_a \cdot \P(Y=-1|Z=a)\label{eqn:fpr}
\end{align}
When $\P(\nY=+1|Z=a) = \P(\nY=+1|Z=b) = 0.5$, we will also have
\begin{align}
   0.5= \P(\nY=+1|Z=a) = \P(Y=+1|Z=a) (1-e_a) + \P(Y=-1|Z=a) e_a 
\end{align}
which returns us that $\P(Y=+1|Z=a) = \frac{0.5 - e_a}{1-2e_a}:=p = 0.5$.
Using this knowledge and solving the linear equations defined by Eqn. (\ref{eqn:tpr}) and (\ref{eqn:fpr}) we have
\begin{align}
    \TPR_a(h) &= \frac{C_{a,1} \cdot \nTPR_a(h) - C_{a,2}\cdot \nFPR_a(h)}{e_a - 0.5 }\\
   \FPR_a(h)&= \frac{C_{a,1} \cdot \nFPR_a(h) - C_{a,2} \cdot \nTPR_a(h)}{e_a - 0.5}
\end{align}

\end{proof}


\subsection{Proof for Theorem \ref{lemma:tpr:violation}}
\begin{proof}
Combining Eqn. (\ref{eqn:fairnesscorrect}) and (\ref{eqn:fairness-estimated}) we have
\begin{align}
    &\ \ |\TPR_z(h)-\TPR^c_z(h)| \nonumber\\
    =&\ \ \left|\frac{0.5 \cdot e_z \cdot \nTPR_z(h) - 0.5(1-e_z)\cdot \nFPR_z(h)}{e_z-0.5}-\frac{0.5 \cdot \widetilde{e}_z \cdot \nTPR_z(h) - 0.5(1-\widetilde{e}_z)\cdot \nFPR_z(h)}{\tilde{e}_z-0.5}\right|\nonumber\\
    =&\ \ \frac{|\tilde{e}_z-e_z| \cdot \nTPR_z(h)}{(2e_z-1)(2\tilde{e}_z-1)}\nonumber \\
   = &\ \ \frac{\texttt{err}_z  \cdot \nTPR_z(h)}{(2e_z-1)(2\tilde{e}_z-1)}~.
    \label{eqn:tpr-diff}
\end{align}
Denote $\texttt{err}_z := |\tilde{e}_z-e_z| $. 
Then equalizing TPR that $\TPR^c_a(h) = \TPR^c_b(h)$ returns us
\begin{align*}
&|\TPR_a(h) - \TPR_b(h)|\\
=&|\TPR_a(h) - \TPR^c_a(h) + \TPR^c_b(h) - \TPR_b(h)|\\
\geq &\left| |\TPR_a(h) - \TPR^c_a(h)| - |\TPR^c_b(h) - \TPR_b(h)| \right|\\
\geq &\left| \frac{\texttt{err}_a \cdot \nTPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)} - \frac{\texttt{err}_b \cdot \nTPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)}\right|,
\end{align*}
where the last inequality is an application of Eqn. (\ref{eqn:tpr-diff}). % Without loss of generality, assume that $\texttt{err}_a \leq \texttt{err}_b$. 
Then 
\begin{align*}
  &  \left| \frac{\texttt{err}_a \cdot \nTPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)} - \frac{\texttt{err}_b \cdot \nTPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)}\right|\\
=&\texttt{err}_a \cdot  \left| \frac{ \nTPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)} - \frac{\texttt{err}_b}{\texttt{err}_a} \frac{\nTPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)}\right|\\
\geq & \errm \cdot  \left| \frac{ \nTPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)} - \frac{\texttt{err}_b}{\texttt{err}_a} \frac{\nTPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)}\right|
\end{align*}

Similarly
\begin{align*}
    &\ \ |\FPR_z(h) - \FPR^c_z(h)|\\
    =&\ \ \left|\frac{0.5 \cdot e_z \cdot \nFPR_z(h) - 0.5(1-e_z)\cdot \nTPR_z(h)}{e_z-0.5}-\frac{0.5 \cdot \widetilde{e}_z \cdot \nFPR_z(h) - 0.5(1-\widetilde{e}_z)\cdot \nTPR_z(h)}{\tilde{e}_z-0.5}\right|\\
    =&\ \ \frac{|\tilde{e}_z-e_z| \cdot \nFPR_z(h)}{(2e_z-1)(2\tilde{e}_z-1)}.
    \\
    = &\ \ \frac{\texttt{err}_z \cdot \nFPR_z(h)}{(2e_z-1)(2\tilde{e}_z-1)}.
\end{align*}
Then equalizing FPR that $\FPR^c_a(h) = \FPR^c_b(h)$ we have
\begin{align*}
&|\FPR_a(h) - \FPR_b(h)|\\
=&|\FPR_a(h) - \FPR^c_a(h) + \FPR^c_b(h) - \FPR_b(h)|\\
\geq &\left| |\FPR_a(h) - \FPR^c_a(h)| - |\FPR^c_b(h) - \FPR_b(h)|\right|\\
\geq &\left| \frac{\texttt{err}_a \cdot \nFPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)} - \frac{\texttt{err}_b \cdot \nFPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)}\right|\\
\geq &\errm \cdot \left| \frac{\nFPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)}  - \frac{\texttt{err}_b}{\texttt{err}_a} \frac{ \nFPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)}\right|.
\end{align*}

% \begin{align*}
% &|\TPR_a(h) - \TPR_b(h)|\\
% =&|\TPR_a(h) - \TPR^c_a(h) + \TPR^c_b(h) - \TPR_b(h)|\\
% \leq &|\TPR_a(h) - \TPR^c_a(h)| + |\TPR^c_b(h) - \TPR_b(h)|\\
% \leq &\frac{\errm \cdot \nTPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)} + \frac{\errm \cdot \nTPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)},
% \end{align*}
% where the last inequality is an application of Eqn. (\ref{eqn:tpr-diff}). Similarly
% \begin{align*}
%     &\ \ |\FPR_z(h) - \FPR^c_z(h)|\\
%     =&\ \ \left|\frac{0.5 \cdot e_z \cdot \nFPR_z(h) - 0.5(1-e_z)\cdot \nTPR_z(h)}{e_z-0.5}-\frac{0.5 \cdot \widetilde{e}_z \cdot \nFPR_z(h) - 0.5(1-\widetilde{e}_z)\cdot \nTPR_z(h)}{\tilde{e}_z-0.5}\right|\\
%     =&\ \ \frac{|\tilde{e}_z-e_z| \cdot \nFPR_z(h)}{(2e_z-1)(2\tilde{e}_z-1)}\\
%     \leq &\ \ \frac{\errm \cdot \nFPR_z(h)}{(2e_z-1)(2\tilde{e}_z-1)}.
% \end{align*}
% Then equalizing FPR that $\FPR^c_a(h) = \FPR^c_b(h)$ we have
% \begin{align*}
% &|\FPR_a(h) - \FPR_b(h)|\\
% =&|\FPR_a(h) - \FPR^c_a(h) + \FPR^c_b(h) - \FPR_b(h)|\\
% \leq &|\FPR_a(h) - \FPR^c_a(h)| + |\FPR^c_b(h) - \FPR_b(h)|\\
% \leq &\frac{\errm \cdot \nFPR_a(h)}{(2e_a-1)(2\tilde{e}_a-1)} + \frac{\errm \cdot \nFPR_b(h)}{(2e_b-1)(2\tilde{e}_b-1)}.
% \end{align*}
\end{proof}



\subsection{Proof for Theorem \ref{thm:fair}}

\begin{proof}
  Easy to show that when $e_a = e_b$, $C_{a,1} = C_{b,1}$ and $C_{a,2} = C_{b,2}$. Therefore, from Eqn. (\ref{eqn:fairnesscorrect}) we know equalizing 
\begin{align}
 \nTPR_a(h) = \nTPR_b(h),~~\nFPR_a(h) = \nFPR_b(h)
\end{align}
will also return us
\begin{align}
 \TPR_a(h) = \TPR_b(h),~~\FPR_a(h) = \FPR_b(h)
\end{align}
\end{proof}

\subsection{Proof for Theorem \ref{thm:detect}}
\begin{proof}
We start with deriving $\PA_{\DS}$. 
\begin{align*}
   \PA_{\DS} =  \P(\nY_2 = \nY_3 = +1|\nY_1 = +1) = \frac{\P(\nY_1 = \nY_2 = \nY_3 = +1)}{\P(\nY_1 = +1)}
\end{align*}
Due to the sampling step, we have $\P(\nY_1 = +1) = 0.5$ - this allows us to focus on the denominator: 
\begin{align*}
    \P(\nY_1 = \nY_2 = \nY_3 = +1) &\stackrel{(1)}{=} \P(Y=+1) \prod_{i=1}^3 \P(\nY_i  = +1|Y=+1) + \P(Y=-1) \prod_{i=1}^3 \P(\nY_i  = +1|Y=-1)\\
    &\stackrel{(2)}{=} \P(Y=+1) \cdot (1-e_+)^3 + \P(Y=-1) \cdot e^3_- 
\end{align*}
where in above, (1) uses the 2-NN clusterability of $D$, and (2) uses the conditional independence between the noisy labels. Similarly for $\NA_{\DS}$ we have:
\begin{align*}
    \P(\nY_2 = \nY_3 = -1|\nY_1 = -1) = \frac{\P(\nY_1 = \nY_2 = \nY_3 = -1)}{\P(\nY_1 = -1)}
\end{align*}
Again we have that $\P(\nY_1 = -1) = 0.5$, and the numerator derives as
\begin{align*}
    \P(\nY_1 = \nY_2 = \nY_3 = -1) &= \P(Y=+1) \prod_{i=1}^3 \P(\nY_i  = -1|Y=+1) + \P(Y=-1) \prod_{i=1}^3 \P(\nY_i  = -1|Y=-1)\\
    &= \P(Y=+1) \cdot e_+^3 + \P(Y=-1) \cdot (1-e_-)^3 
\end{align*}
Taking the difference (and normalize by 0.5) we have
\begin{align}
    &\ \ 0.5 \cdot (\PA_{\DS} - \NA_{\DS})\nonumber\\
    = &\ \ \P(\nY_2 = \nY_3 = +1|\nY_1 = +1) - \P(\nY_2 = \nY_3 = -1|\nY_1 = -1)\nonumber\\
    = &\ \ \P(Y=+1)\left((1-e_+)^3 -  e_+^3 \right) + \P(Y=-1) \left(e^3_- - (1-e_-)^3\right)
    \label{eqn:diff}
\end{align}
Notice two facts: first we can derive that
\begin{align*}
    (1-e_+)^3 -  e_+^3  &= (1-2e_+)(e^2_+ - e_+ + 1),~~e^3_- - (1-e_-)^3 = -(1-2e_-)(e^2_- - e_- + 1)
\end{align*}
Second, we will use the following fact:
\begin{align}
0.5 = \P(\nY = +1) = \P(Y=+1)(1-e_+) + \P(Y=-1) e_-
\end{align}
from which we solve that $\P(Y=+1) = \frac{0.5-e_-}{1-e_+-e_-}$. Symmetrically, $\P(Y=-1) = \frac{0.5-e_+}{1-e_+-e_-}$. 

Return the above two facts back into Eqn. (\ref{eqn:diff}), we have
\begin{align*}
    &\ \ \P(Y=+1)((1-e_+)^3 -  e_+^3 ) +  \P(Y=-1) (e^3_- - (1-e_-)^3)\\
    = &\ \ 2\cdot \frac{(0.5-e_+)(0.5-e_-)}{1-e_+-e_-}\left( (e^2_+ - e_+ + 1) -(e^2_- - e_- + 1) \right)\\
    = &\ \ 2\cdot (0.5-e_+)\cdot (0.5-e_-)\cdot (e_- - e_+)
\end{align*}
completing the proof when $e_+,e_- < 0.5$.
\end{proof}




\subsection{Proof for Proposition \ref{prop:flip}}

\begin{proof}
Expanding $\P(\hat{Y} = -1|Y=+1)$ using the law of total probability we have
 \begin{align*}
\hat{e}_+ &=   \P(\hat{Y} = -1|Y=+1) \\
& = \P(\hat{Y} = -1,\nY=+1|Y=+1)+ \P(\hat{Y} = -1,\nY=-1|Y=+1)\\
    & = \P(\hat{Y} = -1|\nY=+1,Y=+1) \cdot \P(\nY=+1|Y=+1)\\
    &\quad + \P(\hat{Y} = -1|\nY=-1,Y=+1) \cdot \P(\nY=-1|Y=+1)\\
    & = \epsilon \cdot (1-e_+) + 1 \cdot e_+ \tag{\text{Independence between $\hat{Y}$ and $Y$ given $\nY$}}\\
    & = (1-e_+)\cdot \epsilon + e_+ 
\end{align*}
Similarly, 
 \begin{align*}
  \hat{e}_- &=    \P(\hat{Y} = +1|Y=-1) \\
  & = \P(\hat{Y} = +1,\nY=+1|Y=-1)+ \P(\hat{Y} = +1,\nY=-1|Y=-1)\\
    & = \P(\hat{Y} = +1|\nY=+1,Y=-1) \cdot \P(\nY=+1|Y=-1)\\
    &\quad + \P(\hat{Y} = +1|\nY=-1,Y=-1) \cdot \P(\nY=-1|Y=-1)\\
    & = (1-\epsilon) \cdot e_-.
\end{align*}
The last equality is again due to the independence between $\hat{Y}$ and $Y$ given $\nY$, as well as the fact that we do not flip the $\nY=-1$ labels so $\P(\hat{Y} = +1|\nY=-1,Y=-1) = 0$. Taking the difference we finish the proof.
\end{proof}


\subsection{Balancing noise for fairness constrained case}\label{app:sec::balance-for-fairness}

Define 
\begin{align}
     \PA_{\DS,a} =  \P_{Z=a}(\nY_2 = \nY_3 = +1|\nY_1 = +1) \\
          \PA_{\DS,b} =  \P_{Z=b}(\nY_2 = \nY_3 = +1|\nY_1 = +1) 
\end{align}
We now claim that $sgn(\PA_{\DS,a}-\PA_{\DS,b}) = -sgn(e_a-e_b)$. We start with deriving $\PA_{\DS,a}$. 
\begin{align*}
   \PA_{\DS,a} =  \P_{Z=a}(\nY_2 = \nY_3 = +1|\nY_1 = +1) = \frac{\P_{Z=a}(\nY_1 = \nY_2 = \nY_3 = +1)}{\P_{Z=a}(\nY_1 = +1)}
\end{align*}
Due to the sampling step, we have $\P_{Z=a}(\nY_1 = +1) = 0.5$ - this allows us to focus on the denominator: 
\begin{align*}
    \P_{Z=a}(\nY_1 = \nY_2 = \nY_3 = +1) &\stackrel{(1)}{=} \P_{Z=a}(Y=+1) \prod_{i=1}^3 \P_{Z=a}(\nY_i  = +1|Y=+1) \\
    &+ \P_{Z=a}(Y=-1) \prod_{i=1}^3 \P_{Z=a}(\nY_i  = +1|Y=-1)\\
    &\stackrel{(2)}{=} \P_{Z=a}(Y=+1) \cdot (1-e_a)^3 + \P_{Z=a}(Y=-1) \cdot e^3_a 
\end{align*}
where in above, (1) uses the 2-NN clusterability of $D$, and (2) uses the conditional independence between the noisy labels. Similarly for $\PA_{\DS,b}$ we have:
\begin{align}
    \PA_{\DS,b} = \frac{\P_{Z=b}(Y=+1) \cdot (1-e_b)^3 + \P_{Z=b}(Y=-1) \cdot e^3_b}{0.5}
\end{align}
Firstly, we will use the following fact for $z \in \{a,b\}$:
\begin{align*}
0.5 =& \P_{Z=z}(\nY = +1) \\
=&  \P_{Z=z}(\nY = +1|Y=+1)\cdot \P_{Z=z}(Y=+1)+\P_{Z=z}(\nY = +1|Y=-1)\cdot \P_{Z=z}(Y=-1)\\
=& \P_{Z=z}(Y=+1)\cdot (1-e_z) + \P_{Z=z}(Y=-1)\cdot e_z
\end{align*}
from which we solve that $\P_{Z=z}(Y=+1) = \frac{0.5-e_z}{1-2e_z} = 0.5$.
Therefore 
\begin{align}
    \PA_{\DS,a} - \PA_{\DS,b} & = (1-e_a)^3- (1-e_b)^3 + e_a^3- e_b^3 \nonumber \\
    & = (e_b - e_a) \left((1-e_a)^2+(1-e_b)^2+(1-e_a)(1-e_b) - e_a^2-e_b^2-e_a e_b \right) \nonumber \\
    & = (e_b - e_a) \left(1-2e_a + 1-2e_b + 1-e_a-e_b \right)
\end{align}
Note that $1-2e_a + 1-2e_b + 1-e_a-e_b > 0$ when $e_a,e_b < 0.5$. This implies that we can use the 2-NN positive agreements $\PA_{\DS,a} - \PA_{\DS,b}$ across groups to compare $e_a$ with $e_b$.


\subsection{Extension to multi-class}\label{app::sec::estimate-multiclass}
As explained at the beginning, our algorithm can largely extend to the multi-class/group setting. The primary requirement of the extension is to extend the definition of $\PA_{\DS}, \NA_{\DS}$ to each label class/group. Consider a multi-class classification problem with $K$ label classes, and the noise rates follow a uniform diagonal model:
\begin{align}
    \P(\tilde{Y}=k|Y=k) = 1-e_k,~~ \P(\tilde{Y}=k'|Y=k) = \frac{e_k}{K-1},~\forall k'\neq k. 
\end{align}
Define
$
    \KA_{\DS,k}:=\P(\nY_2 = \nY_3 = k|\nY_1 = k), ~k=1,2,...,K
$. Similarly we can show that for any pair of $k_1,k_2$:
$
    sgn(\KA_{\DS,k_1} - \KA_{\DS,k_2}) = - sgn (e_{k_1} - e_{k_2}),
$
wherein above $e_{k_1}, e_{k_2}$ are the error rates of label class $k_1,k_2$. With the above, we can compute $\KA_{\DS,k}$, rank them, and start inserting noise to the classes that are determined to have a lower error rate to match the highest one.

\subsection{Pseudocodes}\label{app::sec::pseudocode}

\begin{figure}[!ht]
\begin{lstlisting}[language=Python]
import numpy as np
from sklearn.neighbors import NearestNeighbors
def estimate_PA(X, y):
    nbrs = NearestNei.(n_neighbors=3, algorithm='ball_tree').fit(X)
    _, indices = nbrs.kneighbors(X)
    return np.mean(np.array([np.all(y[i] == y[indices[i]]) for i in np.where(y > 0)[0]]))
\end{lstlisting}
\vspace{-0.3in}
\caption{\textbf{Numpy-like pseudocode for an implementation of estimating $\PA$.} Our implementation utilizes scikit-learn's Nearest Neighbors module. The code for esimating $\NA$ is similar.}\label{fig:estimate-PA}
\end{figure}

==> can less be more-cr/checklist.tex <==
\newpage
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{One goal of our proposed method aims to improve fairness guarantees when training with noisy labels. The development of the paper is fully aware of any fairness concerns and we believe that applying our methods \textit{thoughtfully} will improve existing methods of bias mitigation in machine learning. Our technical solutions and solvers should be of interests to machine learning practitioners/researchers, as well as to policy makers when decided to use classification tools but face a training data with low-quality annotations. We are not aware of any negative societal impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We have the full details in the Appendix (supplementary material). }
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have included the details and codes in our supplementary material. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> can less be more-cr/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> checklist.tex <==
\newpage
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{One goal of our proposed method aims to improve fairness guarantees when training with noisy labels. The development of the paper is fully aware of any fairness concerns and we believe that applying our methods \textit{thoughtfully} will improve existing methods of bias mitigation in machine learning. Our technical solutions and solvers should be of interests to machine learning practitioners/researchers, as well as to policy makers when decided to use classification tools but face a training data with low-quality annotations. We are not aware of any negative societal impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We have the full details in the Appendix (supplementary material). }
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have included the details and codes in our supplementary material. }
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

